Effective Non-oscillatory Regularized L$_1$ Finite Elements for Particle Transport Simulations

In this work, we present a novel regularized L$_1$ (RL$_1$) finite element spatial discretization scheme for radiation transport problems. We review the recently developed least-squares finite element method in nuclear applications. We then derive an L$_1$ finite element by minimizing the L$_1$ norm of the transport residual. To ensure the stability on incident boundary, we newly develop a consistent L$_1$ boundary condition (BC). The numerical tests demonstrate such a method effectively prevents the oscillations which would occur to least-squares finite element when discontinuity exists such as void and absorber. Further, the RL$_1$ method is accurate in problems with scattering.

==> packages.tex <==
%  various packages that you may wish to activate for usage
\usepackage{graphicx}
\usepackage{tabls}
\usepackage{afterpage}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amstext}
\usepackage{amsbsy}
\usepackage{epsfig}
%\usepackage{cites}
\usepackage{epsf}
\usepackage{float} %utiliser H pour forcer à mettre l'image où on ve

\usepackage{array}
{\usepackage{xcolor}}
\usepackage[section]{placeins} % force à mettre l'image où on veut
\usepackage{lscape} %utilisation du mode paysage
\usepackage{xspace}

%\usepackage[pdftex,bookmarks=true]{hyperref}
\usepackage{url}
\usepackage{verbatim}
%\usepackage[all]{hypcap}

\usepackage[labelsep=quad]{caption} % needed by the breakalgo environment

\usepackage{ifthen}
%\usepackage{subfig}

\usepackage{ulem}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{listings}
\usepackage[noprefix]{nomencl}  % for nomenclature
%\usepackage[intoc]{nomencl}  % for nomenclature

%\usepackage{notebook2e, latexsym}
%
% de dk:
%
%%\usepackage[dvips]{epsfig}
%%\usepackage[dvips]{graphicx}
%%\usepackage{comment}
%%\usepackage{floatfig}
%%\usepackage{lscape}
%%\usepackage{landscape}
%%\usepackage{graphics}
%%\usepackage{hhline}[]
%%\usepackage{latexsym}
%%\usepackage{tabularx}[]
%%\usepackage{layout}
%
% de btp:
%
%%\usepackage{fancyheadings}
%%\usepackage{minitoc}
\usepackage{rotating}
%% \usepackage{rotate}
%\usepackage{subfigure}
\usepackage{subcaption}
%%\usepackage{mathaccent}
%%\usepackage{isolatin1}
%
%%\usepackage{xspace}
%%\usepackage{longtable}
%%\usepackage{caption2}
%%\usepackage{ifthen}
%
\usepackage{mathpazo}
\usepackage{hyperref}
%\usepackage{spconf}
\usepackage{stmaryrd}

